What Do We Mean When We Talk About Infographics?

There has been limited clarity and consistency regarding what the term infographics, or information graphics, refers to in visualization research and practice. In particular, little is understood about where people's conceptualizations of infographics converge or diverge. To address this gap, we conducted a systematic literature review and a practitioner survey to identify and contrast different perspectives on infographics. We performed inductive coding on 487 sentences from 111 visualization and HCI papers, and analyzed questionnaire responses from 44 domain practitioners. Our findings reveal recurring dimensions of conceptual disagreement on infographics: role of text, relationship with data visualization, and relationships with statistical charts and data comics. Based on the results, we recommend future work to explicitly report any assumptions made along these diverging conceptualizations, to investigate the cognitive origins of these disagreements, and to develop more holistic design component frameworks for infographics. The supplementary materials are available via OSF and as an interactive web application.

==> sec/import.tex <==
\usepackage{amsmath,amssymb}
\usepackage{fontawesome5}
\usepackage{cite}
\RequirePackage[nameinlink,capitalise]{cleveref}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}

\usepackage{multirow}
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{soul}

\newcommand{\circled}[1]{\protect\tikz[baseline=(char.base)]{\protect\draw circle [radius=5px] node (char) {#1}}}
\newcommand{\btn}[1]{\protect\tikz[baseline=0.5px]{\protect\fill[#1, rounded corners=1px] (0,0) rectangle (0.8em, 0.8em)}}
\newcommand{\ptn}[1]{\protect\tikz[baseline=-2.8px]{\protect\fill[#1] (0,0) circle (0.3em)}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\outline}[1]{\fbox{#1}}

\definecolor{masuhana}{HTML}{577C8A}
\definecolor{subset}{HTML}{FCE5CD}
\definecolor{superset}{HTML}{FFF2CC}
\definecolor{equal}{HTML}{D9EAD3}
\definecolor{intersect}{HTML}{F3F3F3}
\definecolor{unequal}{HTML}{D9D2E9}
\definecolor{unknown}{HTML}{E6B8AF}

\newcommand{\abbr}{...~}
\newcommand{\textor}{\,/\,}
\newcommand{\andor}{and\textor or }
\newcommand{\andorx}{and\textor or}
\newcommand{\ig}{infographics }
\newcommand{\igx}{infographics}
\newcommand{\igc}{infographic }
\newcommand{\igcx}{infographic}
\newcommand{\Ig}{Infographics }
\newcommand{\Igx}{Infographics}
\newcommand{\Igc}{Infographic }
\newcommand{\Igcx}{Infographic}
\newcommand{\igr}{information graphics }
\newcommand{\igrx}{information graphics}
\newcommand{\etal}{et~al.~}
\newcommand{\etalx}{et~al.}

\newcommand{\flatquote}[1]{``#1''}
\renewcommand{\quote}[1]{\flatquote{\emph{#1}}}
\newcommand{\quotealt}[1]{\textnormal{[}#1\textnormal{]}}
\newcommand{\parsec}[1]{\noindent\textbf{#1.}}
\newcommand{\parseq}[1]{\textbf{#1?}}
\newcommand{\study}[1]{Study~#1}
\newcommand{\combine}{\,+\,}

\newcommand{\osf}{\href{https://osf.io/yuqjn/overview}{OSF}}

\newcommand{\app}{\href{https://talk-about-infographics.netlify.app/}{interactive web application}}
\newcommand{\appnote}{\footnote{These files are also hosted at \app, under \flatquote{Data Download.} Datasets are provided here in XLSX format for ease of viewing; for the equivalent CSV versions, please visit the URL above.}}

\definecolor{def}{HTML}{ae82e0}
\definecolor{ex}{HTML}{72b8ce}
\definecolor{cmp}{HTML}{f5ad42}

\newcommand{\typea}{\colortag{def}{DEF}}
\newcommand{\typeb}{\colortag{ex}{EX}}
\newcommand{\typec}{\colortag{cmp}{CMP}}

\newcommand{\counticon}[1]{\raisebox{0.4pt}{\faIcon[regular]{#1}}}
\newcommand{\countl}{\colortag{gray}{\counticon{file}}}
\newcommand{\countp}{\colortag{gray}{\counticon{user}}}

\newcommand{\nx}[3]{\textcolor{#1}{\small\sf #2}\,#3}
\newcommand{\na}[1]{\nx{def}{#1}{\typea}}
\newcommand{\nb}[1]{\nx{ex}{#1}{\typeb}}
\newcommand{\nc}[1]{\nx{cmp}{#1}{\typec}}
\newcommand{\nl}[1]{\nx{gray}{#1}{\countl}}
\newcommand{\np}[1]{\nx{gray}{#1}{\countp}}

\definecolor{Design}{HTML}{666666}
\definecolor{Goal}{HTML}{666666}
\definecolor{Content}{HTML}{666666}
\definecolor{Authoring}{HTML}{666666}
\definecolor{Application}{HTML}{666666}
\definecolor{Comparison}{HTML}{666666}

\newcommand{\from}{\raisebox{1.5px}{\scalebox{0.6}{$\blacktriangleleft$}}}
\newcommand{\ptr}{\raisebox{1.5px}{\scalebox{0.6}{$\blacktriangleright$}}}
\newcommand{\aspect}[1]{\ptn{#1}~#1}
\newcommand{\group}[2]{{\small\textcolor{#1}{\sf{#1}\;$\rightarrow$\,\sf{#2}}}}
\newcommand{\codetext}[1]{\textbf{\emph{#1}}}
\newcommand{\code}[4]{\parsec{#1} (#2) #4}
\newcommand{\codefrom}[3]{#1; \nl{#2}, \np{#3}}
\newcommand{\codefroml}[2]{#1; \nl{#2}}
\newcommand{\term}[1]{\textbf{$\langle\text{#1}\rangle$}}

\newcommand{\related}[1]{\textbf{#1} (Relation: \codetext{related})}
\newcommand{\contrary}[1]{\textbf{#1} (Relation: \codetext{contrary})}
\newcommand{\relcon}[1]{\textbf{#1} (Relation: \codetext{related}, \codetext{contrary})}

\newcommand{\file}[1]{\item[$\blacktriangleright$] \underline{\texttt{#1}}}
\newcommand{\field}[1]{\textcolor{cyan!50!blue}{\texttt{#1}}}
\newcommand{\markx}{\field{\textquotesingle x\textquotesingle}}
\newcommand{\syn}[2]{#1\,$\Leftrightarrow$\,#2}

